Fairness in Machine Learning meets with Equity in Healthcare

With the growing utilization of machine learning in healthcare, there is increasing potential to enhance healthcare outcomes. However, this also brings the risk of perpetuating biases in data and model design that can harm certain demographic groups based on factors such as age, gender, and race. This study proposes an artificial intelligence framework, grounded in software engineering principles, for identifying and mitigating biases in data and models while ensuring fairness in healthcare settings. A case study is presented to demonstrate how systematic biases in data can lead to amplified biases in model predictions, and machine learning methods are suggested to prevent such biases. Future research aims to test and validate the proposed ML framework in real-world clinical settings to evaluate its impact on promoting health equity.

==> figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

%%%%%%%%%%%%% Figure 1
\begin{figure}
\centering
\begin{subcaptiongroup}
\phantomcaption\label{fig:1A} % add one of these for each subpanel
\phantomcaption\label{fig:1B} % add one of these for each subpanel
\end{subcaptiongroup}
\includegraphics[width=1\textwidth]{figures/sampfig.png}
\caption{\textcolor{Highlight}{\textbf{Schematic illustrations of apparatus design.}}\\
(A)
Some text.\\
(B)
More text.\\
(C) 
Last text.
}
\label{fig:F1}

\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUPPLEMENTAL Figures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\beginsupplement % <- renumbers everything and starts figure naming with "S" per local.sty

==> table.tex <==
\begin{table}
\captionsetup{margin={0.5in,0in}} % nudge the first number to move the caption over to match the table width
\caption{\textcolor{Highlight}{Table caption} Table caption text here}
\centering
\begin{small}
\begin{tabular}{p{0.125\textwidth}M{0.1\textwidth}M{0.15\textwidth}M{0.1\textwidth}M{0.1\textwidth}M{0.125\textwidth}}

\toprule

\textbf{A}  & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E} & \textbf{F} \\
\midrule
        &     &    &    &    &    \\
A type  &     &    &    &    &    \\
\midrule
I       & 1  &    &    &    &    \\
II      & 2  &    &    &    &    \\
III     & 3  &    &    &    &    \\
IV      & 4  &    &    &    &    \\
 &     &    &    &    &    \\
Totals:   & 10 & 0 & 0 & 0 & 0\\
\bottomrule
\end{tabular}
\end{small}
\label{tab:1}
\end{table}

